NovelCraft: A Dataset for Novelty Detection and Discovery in Open Worlds

In order for artificial agents to successfully perform tasks in changing environments, they must be able to both detect and adapt to novelty. However, visual novelty detection research often only evaluates on repurposed datasets such as CIFAR-10 originally intended for object classification, where images focus on one distinct, well-centered object. New benchmarks are needed to represent the challenges of navigating the complex scenes of an open world. Our new NovelCraft dataset contains multimodal episodic data of the images and symbolic world-states seen by an agent completing a pogo stick assembly task within a modified Minecraft environment. In some episodes, we insert novel objects of varying size within the complex 3D scene that may impact gameplay. Our visual novelty detection benchmark finds that methods that rank best on popular area-under-the-curve metrics may be outperformed by simpler alternatives when controlling false positives matters most. Further multimodal novelty detection experiments suggest that methods that fuse both visual and symbolic information can improve time until detection as well as overall discrimination. Finally, our evaluation of recent generalized category discovery methods suggests that adapting to new imbalanced categories in complex scenes remains an exciting open problem.

==> Makefile <==
## To build paper PDF: 'make main.pdf'

SHELL=/bin/bash

MAIN?=main

TMP_RESULT=$$(bash -c "find . -name '*.tex' -maxdepth 2 | xargs grep "figures/" | cut -d':' -f2 | grep -v '%'");
PDF_FIG_FILES=$$(python -c "print(' '.join([s + ('.pdf' * (1 - s.endswith('.pdf')) * (1 - s.endswith('.png'))) for s in [x.partition('}')[0] for x in '''${TMP_RESULT}'''.split('{')] if s.startswith('figures/')]))")

PNG_FIG_FILES=$$(python -c "print(' '.join([s for s in [x.partition('}')[0] for x in '''${TMP_RESULT}'''.split('{')] if s.startswith('figures/') and s.endswith('.png') ]))")

#ALL_FIG_FILES="${PDF_FIG_FILES} ${PNG_FIG_FILES}"

OUTPUTFILE_DOCX?=$(MAIN).docx
BIBLIO_OPTS = --bibliography *.bib --csl apa.csl

all: $(MAIN).pdf $(MAIN).docx

clean:
	rm -fv *.zip *.aux *.log *.bbl *.blg *.ptc *.toc *.out *.lot *.lof *.dvi *.ps *.pdf *.docx

clean_extras:
	rm -fv *.aux *.bbl *.blg *.toc *.out *.lot *.lof

pdf: $(MAIN).pdf

paper: $(MAIN).pdf

$(MAIN).pdf: $(MAIN).bbl *.tex
	# Run 3x to get cross refs right
	pdflatex -interaction nonstopmode $(MAIN) || true
	pdflatex -interaction nonstopmode $(MAIN) || true
	pdflatex -interaction nonstopmode $(MAIN) || true
	pdflatex -interaction nonstopmode $(MAIN) && make clean_extras

$(MAIN).bbl: $(MAIN).tex *.tex *.bib
	pdflatex -interaction nonstopmode $(MAIN) || true
	bibtex $(MAIN) && rm main.pdf

$(OUTPUTFILE_DOCX): *.tex *.bib figures/*.pdf
	pandoc $(MAIN).tex \
		--from latex \
		--to docx \
		--output $(OUTPUTFILE_DOCX) \
		$(BIBLIO_OPTS)

src_for_arxiv.zip: $(MAIN).bbl $(MAIN).tex *.tex *.bib
	zip -r src_for_arxiv.zip \
		*.bbl \
		jmlr_arxiv.cls \
		jmlrutils.sty \
		abbrvnat_maxauthors8.bst \
		*.tex \
		$(PDF_FIG_FILES) \
		$(PNG_FIG_FILES)


==> checklist.tex <==
%%% BEGIN INSTRUCTIONS %%%
%The checklist follows the references.  Please
%read the checklist guidelines carefully for information on how to answer these
%questions.  For each question, change the default \answerTODO{} to \answerYes{},
%\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
%justification to your answer}, either by referencing the appropriate section of
%your paper or providing a brief inline description.  For example:
%\begin{itemize}
%  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%  \item Did you include the license to the code and datasets? \answerNA{}
%\end{itemize}
%Please do not modify the questions and only use the provided macros for your
%answers.  Note that the Checklist section does not count towards the page
%limit.  In your paper, please delete this instructions block and only keep the
%Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{The claims in the abstract and introduction are specific and supported by empirical evidence in the results.}
  \item Did you describe the limitations of your work?
    \answerYes{See the paragraph in Sec.~\ref{sec:discussion}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{Potential negative societal impacts are discussed in Section~\ref{sec:discussion}.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{We have ensured that our paper conforms to the General Ethical Conduct and Potential Negative Social Impacts guidelines.}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{No theoretical results included.}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{No theoretical results included.}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Data is available at \datasetURL. Code and instructions to reproduce experimental results, as well as the model outputs used to generate data labels, figures, and tables, are available at \codeURL.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Data splits and an overview of hyperparameters and the searches done are included in the paper. Detailed information is available in the supplement and code repository.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{Error bars were not included due to the cost of training models multiple times. Our results are generally very clearly separated. One exception is when all tested models are roughly equivalent as in TNR at PPV 80\% in Table~\ref{tab:results_detect_visual}. We have code neccessary to produce error bars via bootstrap resampling of the test set if reviewers request it.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{Compute resources used for each method are included in the supplement.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We cite the creator of both the simulation environment and the agent utilized during data collection.}
  \item Did you mention the license of the assets?
    \answerNA{None of the existing assets have a specific license that is publicly known, but we did get explicit written permission from the creators to use these assets to create and release our work. We have made the licenses of our released assets clear on page 1.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{New assets are provided via URL.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{Our work uses existing assets used with permission of the creators, not data tied to specific people.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{Our work does not include data about people.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{No crowdsourcing or human subject research.}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{No crowdsourcing or human subject research.}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{No crowdsourcing or human subject research.}
\end{enumerate}

\end{enumerate}


==> fig_data_placeholder.tex <==
\begin{figure}[!h]
\begin{tabular}{c c}
\begin{minipage}{.6\textwidth}
\setlength{\tabcolsep}{0.05cm} % squeeze cols together
STUFF HERE
\end{minipage}
&
\begin{minipage}{.4\textwidth}
\begin{lstlisting}[language=json,firstnumber=1]
{"map": {
"45,17,52": {
  "name": "plastic_chest",
  "isAccessible": true,
  "facing": "north"
},
"47,17,56": {
  "name": "log",
  "isAccessible": true,
  "axis": "y",
  "variant": "oak"
},
"59,17,62": {
  "name": "air",
  "isAccessible": true
}
...
}}
\end{lstlisting}
\end{minipage}
\end{tabular}
%\caption{Example JSON formatting for mapping positions to object data. Each frame in our dataset contains JSON data for all objects and environment-controlled agents. Additionally data about player state and agent actions is included.
%}%endcaption
%\label{fig:json_symbolic_example}
%\end{figure}
\caption{
Examples from our new multi-modal \datasetName~dataset.
\textbf{\emph{Left:}} Images from different episodes, two normal (rows 1-2) and two novel (rows 3-4).
Only a few images in the novel episodes (highlighted in red) actually contain novel content, making detection challenging.
\textbf{\emph{Right:}} Example symbolic information from one frame, indicating for each 3D position on the map the name and properties of the object in that position.
At each frame, we record a complete JSON representation of all objects and other artificial agents in the world.
Data about player state and agent actions is also included.
}%endcaption
\label{fig:motivation_with_example_images}
\end{figure}


==> fig_json_example_symbolic.tex <==
\begin{figure}[!h]
% TODO what can we include side-by-side with this figure?
\begin{minipage}{.7\textwidth}
\begin{lstlisting}[language=json,firstnumber=1]
{"map": {
    "45,17,52": {
      "name": "polycraft:plastic_chest",
      "isAccessible": true,
      "facing": "north"
    },
    "47,17,56": {
      "name": "minecraft:log",
      "isAccessible": true,
      "axis": "y",
      "variant": "oak"
    },
    "59,17,62": {
      "name": "minecraft:air",
      "isAccessible": true
    }
}}
\end{lstlisting}
\end{minipage}
\caption{Example JSON formatting for mapping positions to object data. Each frame in our dataset contains JSON data for all objects and environment-controlled agents. Additionally data about player state and agent actions is included.
}%endcaption
\label{fig:json_symbolic_example}
\end{figure}


==> tasks.tex <==


\subsection{Symbolic Novelty Detection Task on \datasetAbbrev}
As indicated in section \ref{sec:dataset}, along with images the environment provides a JSON file that fully specifies the state of the environment at each time-step. Using that information, we create another novelty detection task that consists of detecting novel state-transitions, which correspond to novel dynamics in the underlying game. While most of our novelties are aimed at visual detection, one novelty also manifests as a novel state transition, so in this task we limit the test set to include all the non-novel samples and all samples from this one novel category. 

We approach the problem of detecting novel state transitions by  selecting entries from the JSON file and modeling them as a multivariate time-series. We train a predictive model that uses a fixed window size over the temporal context and use the average prediction error over the episode as a novelty signal. 

\paragraph{Predictive Model. } The architecture of our predictive model is a simple multi-layer perceptron with 1 hidden layer with a hidden dimension of size 64. The model uses a temporal context of 5 time-steps. We train the model for 30 epochs with early stopping based on the validation loss. We use a learning rate of $10^{-4}$ with the Adam optimizer.  






\subsection{Candidate Methods for Symbolic Detection}



\subsection{Novelty Characterization Task on \datasetAbbrev}

\subsection{Candidate Methods for Novelty Characterization}


